SALA: Soft Assignment Local Aggregation for Parameter Efficient 3D Semantic Segmentation

In this work, we focus on designing a point local aggregation function that yields parameter efficient networks for 3D point cloud semantic segmentation. We explore the idea of using learnable neighbor-to-grid soft assignment in grid-based aggregation functions. Previous methods in literature operate on a predefined geometric grid such as local volume partitions or irregular kernel points. A more general alternative is to allow the network to learn an assignment function that best suits the end task. Since it is learnable, this mapping is allowed to be different per layer instead of being applied uniformly throughout the depth of the network. By endowing the network with the flexibility to learn its own neighbor-to-grid assignment, we arrive at parameter efficient models that achieve state-of-the-art (SOTA) performance on S3DIS with at least 10$\times$ less parameters than the current reigning method. We also demonstrate competitive performance on ScanNet and PartNet compared with much larger SOTA models.

==> tables/ablations.tex <==
\begin{table}[t]
    \small
    \tabcolsep=0.13cm
    \begin{center}
        \begin{tabular}{l|c|c}
            \hline
            Method & SALA Input & S3DIS A5\\
            \hline
            PointNet++ \cite{pointnet++} & $[p_{ij},f_j]$ & -\\
            PointwiseMLP (C=36, 1.6M) \cite{closerlook3d} & $[p_{ij},f_i, f_{ij}]$ & 56.7\\
            PointwiseMLP (C=144, 25.5M) \cite{closerlook3d} & $[p_{ij},f_i, f_{ij}]$ & 66.2\\
            \hline
            1 group - SALANet (C=36, 1.4M) & $[r_j,f_j]$ & 65.5\\
            2 groups - SALANet$^\mathbf{+}$ (C=36, 1.6M) & $[r_j,f_j]$ & \textbf{67.6}\\
            3 groups - SALANet (C=36, 1.8M) & $[r_j,f_j]$ & 65.7\\
            \hline
            \hline
            1 group - SALANet (C=36, 1.4M) & $[p_{ij},f_j]$ & 61.1\\
            1 group - SALANet (C=36, 1.5M) & $[p_{ij},f_i, f_{ij}]$ & 65.1\\
            2 groups - SALANet (C=36, 1.6M) & $[p_{ij},f_j]$ & 65.5\\
            2 groups - SALANet (C=36, 1.8M) & $[p_{ij},f_i, f_{ij}]$ & 66.4\\
            \hline
        \end{tabular}
        \vspace{1pt}
        \caption{\textbf{Ablation of SALANet on S3DIS Area $5$}. We report results of SALANet model variants using SALA with different numbers of groups and different 
        aggregation inputs  ($f^*_j$) on S3DIS test Area $5$ (A5). The upper table sub-part corresponds to varying the number of groups and the lower sub-part corresponds to varying the choice of inputs. (+) denotes the configuration of choice. $\mathbf{M}$ corresponds to million parameters.}\label{table:ablation}
        \end{center}
\end{table}

==> tables/ablations3.tex <==
\begin{table}[t]
    \small
    \tabcolsep=0.3cm
    \begin{center}
        \begin{tabular}{l|c}
            \hline
            Method & S3DIS A5 (mIoU)\\
            \hline
            Point-wise MLP (C=36, 1.6M) \cite{closerlook3d} & 56.7\\
            Adapt Weights (C=36, 1.2M)\cite{closerlook3d} & 61.9\\
            Pseudo Grid (C=36, 1.2M)\cite{closerlook3d} & 64.3\\
            PosPool (C=36, 1.1M)\cite{closerlook3d} &  64.2\\
            KPConv (r) (14.1M)\cite{kpconv} & 65.4\\
            \hline
            2 groups - SALANet (C=18, 0.41M) & 64.9\\
            \hline
        \end{tabular}
        \vspace{3pt}
        \caption{\textbf{Smaller SALANet on S3DIS Area $5$}. We explore even smaller SALANet model with 0.41M parameters that outperforms models with at least 3 $\times$ more parameters, and is on par with model with 34 $\times$ less parameters. $\mathbf{M}$ corresponds to million parameters.}\label{table:ablation3}
        \end{center}
\end{table}

==> tables/comparison.tex <==
\begin{table*}[htb]
    \small
    \tabcolsep=0.07cm
    \begin{center}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l  | c | c c c c c c c c c c c c c}
            \hline
            Method & mIoU & ceiling & floor & wall & beam & column & window & door & table & chair & sofa & book. & board & clutter \\
            \hline
            KPConv (r) (14.1M)\cite{kpconv} & 65.4  & 92.6  & 97.3  & 81.4  & 0 & 16.5 & 54.5 & 69.5 & 80.2 & 90.1 & 66.4 & 74.6 & 63.7 & 58.1  \\
            KPConv (d) (14.9M)\cite{kpconv} & 67.1 & 92.8 & 97.3 & 82.4 & 0 & 23.9 & 58 & 69 & 81.5 & 91 & 75.4  & 75.3  & \textbf{66.7}  & 58.9  \\
            \hline
            \hline
            1 group - SALANet (1.4M) & 65.5 & \textbf{95.5} & 98.3 & 81.5 & 0 & 9.2  & 56.3  & 63.1 & 82.1 & 89.9 & \textbf{75.5} & 75.5 & 62.2 & \textbf{62}    \\
            2 groups - SALANet$^\mathbf{+}$ (1.6M)   & \textbf{67.6} & 94.9 & \textbf{98.3} & \textbf{82.5} & 0 & \textbf{26.2} & 55 & \textbf{71.1} & \textbf{82.7} & \textbf{91.3} & 73.3 & \textbf{77.8} & 63.8 & 61.9 \\
            % 3 groups - SALANet (1.8M) & 65.7 & 94.8 & 98.3 & 82.5 & 0 & 11.5 & \textbf{58.1} & 66.9 & 82.2 & 90.5 & 67.1 & 76.4 & 63.0 & 62.5 \\
            \hline
        \end{tabular}}
        \vspace{1pt}
        \caption{\textbf{Comparison with KPConv on S3DIS Area 5.} We compare the per class IoU of KPConv \cite{kpconv} against that of SALANet with different group kernel settings. (+) denotes the configuration of choice. $\mathbf{M}$ corresponds to million parameters.
        }\label{table:comparison}
    \end{center}
\end{table*}
